StableToolBench: Towards Stable Large-Scale Benchmarking on Tool Learning of Large Language Models

Large Language Models (LLMs) have witnessed remarkable advancements in recent years, prompting the exploration of tool learning, which integrates LLMs with external tools to address diverse real-world challenges. Assessing the capability of LLMs to utilise tools necessitates large-scale and stable benchmarks. However, previous works relied on either hand-crafted online tools with limited scale, or large-scale real online APIs suffering from instability of API status. To address this problem, we introduce StableToolBench, a benchmark evolving from ToolBench, proposing a virtual API server and stable evaluation system. The virtual API server contains a caching system and API simulators which are complementary to alleviate the change in API status. Meanwhile, the stable evaluation system designs solvable pass and win rates using GPT-4 as the automatic evaluator to eliminate the randomness during evaluation. Experimental results demonstrate the stability of StableToolBench, and further discuss the effectiveness of API simulators, the caching system, and the evaluator system.

==> sections/4_exps.tex <==
\subsection{Experimental Setups}

% \subsection{Query Construction}
% \textcolor{red}{Discussion: Position of query construction in the paper.}
% % Curating a large number of real-world queries based on a large-scale tool set is a non-trival problems. To balance 

% In addition to the original queries in ToolBench, we further create queries aiming at improved reality and quality of benchmark. In ToolBench, queries are created from the bottom-up, i.e., LLMs will write questions based on the APIs they are given. In this way, although the feasibility of the queries is guaranteed, reality is sacrificed. This is because when it comes to more complex multi-step questions, LLMs may connect unrelated APIs to make up an unnatural query. For example, in the following query: 

%  \texttt{I'm working on a project and I need some data related to addresses in Brazil. Can you provide me with address details using the postal code 75094080? Also, I would like to know the health status of the SQUAKE API.}

% \noindent The first and the second subquery, asking for address details and API status are not related.

% To enhance the reality of the queries, we further create some queries with cluster APIs functionalities with specified scenarios. Specifically, we first extract some scenarios from the training set of the ToolBench dataset, by prompting \texttt{GPT-4}. Then, we encode all tools by their documentation using \texttt{E5-Mistral-7B-Instruct}~\cite{wang2022text, wang2023improving}, following EasyTool~\cite{yuan2024easytool}. We cluster these APIs with K-Means~\cite{MacQueen1967SomeMF}. Within each cluster, we summarise the functionality of this cluster with \texttt{GPT-3.5-Turbo}. At last, for each scenario, we retrieve the top 5 clusters of APIs by the cosine similarity between the scenarios and the cluster centres and then ask GPT-4 to write queries based on the scenarios and retrieved clusters. Based on the clustered APIs, the detailed functionality of the APIs is blurred, allowing more natural queries.









==> sections/5_ablation.tex <==
\subsection{Ablation studies}
\textcolor{red}{Analyse the impact of simulation and cache on the stability}
